Forecasting the Evolution of Hydrogen Vehicle Fleet in the UK usingGrowth and Lotka-Volterra Models

Road vehicles play an important role in the UK's energy systems and are a critical component in reducing the reliance on fossil fuels and mitigating emissions. A dynamic model of vehicle fleet, based on predator-prey concepts, is presented. It allows to predict the evolution of the hydrogen based vehicle's role in the UK's vehicle fleet and the sensitivity of this growth to the supply chain. In addition to this, this model is used to predict the demand of hydrogen for the passenger vehicle fleet for various scenarios. A key result is that the amount of hydrogen required to support a huge network of hydrogen based vehicles is currently not practical, regarding the infrastructure required and the cost to build such an infrastructure. In order to mitigate that, the policy focus should move primarily from hydrogen based vehicles to first encompass range extenders in the transport energy system.

==> tikz/first_order.tex <==
\input{./tikz/tikz_preamble}
\begin{tikzpicture} 
    \begin{axis}[
        height = .40\linewidth,
        width = .50\linewidth,
        legend pos=north west,
        legend style={fill=white, fill opacity=0.5, draw opacity=1,text opacity=1},
        xlabel={Time since 1950,
        ylabel={Number of vehicles (millions)},
        %ytick = {1.e3,1.e4,1.e6},
        %xtick = {.1,.5,1,5},
        %xmin=1970,xmax=2020,
        %ymin=50,ymax=2e6,
        ]
        %
        %
        \addplot[mark=o,color=red,solid] 
            coordinates{
            (1,1263.6)
            (2,2572.2)
            (3,3790.8)
            (4,5053.5)
            (5,6317.1)
            (10,12634.2)
            (20,25269.3)
            (30,37903.5)
            (40,50538.6)
            (50,63172.8)
            (100,126346.5)
            };
        \addplot[mark=x,color=black,very thick,dashed]
            coordinates{
                (1,1263)
                (10,12630)
                (100,126300)
            };
    \end{axis}
\end{tikzpicture}


==> tikz/growth_data.tex <==
\input{./tikz/tikz_preamble}
\begin{tikzpicture} 
    \begin{axis}[
        height = .40\linewidth,
        width = .50\linewidth,
        legend pos=north west,
        legend style={fill=white, fill opacity=0.5, draw opacity=1,text opacity=1},
        xlabel={year},
        ylabel={car park (millions)},
        %ytick = {1.e-3,1.e-1,10},
        %xtick = {.1,.5,1,5},
        xmin=1970,xmax=2020,
        %ymin=1.e-3,ymax=10,
        ]
        %
        %
        \addplot[mark=x,color=red,solid,very thick] 
            coordinates{
            (1971,8)
            (1976,10)
            (1981,10)
            (1986,13)
            (1991,16)
            (1996,18)
            (2001,20)
            (2006,25)
            (2011,27)
            (2016,29)
            };
        \addplot[mark=none,color=red,solid,domain=1970:2020,samples=50] {0.4921*x - 963.44}; 
        
    \end{axis}
\end{tikzpicture}


==> tikz/rs_data.tex <==
\input{./tikz/tikz_preamble}
\begin{tikzpicture} 
    \begin{axis}[
        height = .40\linewidth,
        width = .50\linewidth,
        legend pos=north west,
        legend style={fill=white, fill opacity=0.5, draw opacity=1,text opacity=1},
        xlabel={Number of Recharge Station},
        ylabel={Number of HFCVs},
        %ytick = {1.e3,1.e4,1.e6},
        %xtick = {.1,.5,1,5},
        %xmin=1970,xmax=2020,
        %ymin=50,ymax=2e6,
        ]
        %
        %
        \addplot[mark=o,color=red,solid] 
            coordinates{
            (1,1263.6)
            (2,2572.2)
            (3,3790.8)
            (4,5053.5)
            (5,6317.1)
            (10,12634.2)
            (20,25269.3)
            (30,37903.5)
            (40,50538.6)
            (50,63172.8)
            (100,126346.5)
            };
        \addplot[mark=x,color=black,very thick,dashed]
            coordinates{
                (1,1263)
                (10,12630)
                (100,126300)
            };
    \end{axis}
\end{tikzpicture}


==> tikz/tikz_preamble.tex <==
% general parameter
\pgfplotsset{compat=newest}
% picture size
\pgfplotsset{height=0.4\linewidth,}
% label format
\pgfplotsset{    
		x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    	y label style={at={(axis description cs:-0.1,.5)},anchor=south},
        ylabel near ticks,
        %xlabel near ticks,
		%ylabel style={overlay, anchor=north,},
		%label style={anchor=near ticklabel},
    	%xlabel style={yshift=0.5em},
    	%ylabel style={yshift=-0.5em},
		ylabel shift = -0.5em,
}
\pgfplotsset{every axis/.append style={
                    legend style={font=\tiny,line width=.5pt,mark size=.6pt},
                    }}
% axis format
\pgfplotsset{
		axis on top,
        xtick align=inside,
        %scale only axis,
        %enlarge x limits=0.05,
        %enlarge y limits=0.05,
}
% cycle
\pgfplotscreateplotcyclelist{newcolors}
{%
blue,           every mark/.append style={fill=blue!80!black},mark=*\\%
red,            every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black, every mark/.append style={fill=brown!80!black},mark=otimes*\\%
black,          mark=star\\%
blue,           every mark/.append style={fill=blue!80!black},mark=diamond*\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
black,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=star,every mark/.append style=solid\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*\\%
}

%axis style when log
\pgfplotsset{
  log x ticks with fixed point/.style={
      xticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  },
  log y ticks with fixed point/.style={
      yticklabel={
        \pgfkeys{/pgf/fpu=true}
        \pgfmathparse{exp(\tick)}%
        \pgfmathprintnumber[fixed relative, precision=3]{\pgfmathresult}
        \pgfkeys{/pgf/fpu=false}
      }
  }
}

